A Nonparametric Off-Policy Policy Gradient

Reinforcement learning (RL) algorithms still suffer from high sample complexity despite outstanding recent successes. The need for intensive interactions with the environment is especially observed in many widely popular policy gradient algorithms that perform updates using on-policy samples. The price of such inefficiency becomes evident in real-world scenarios such as interaction-driven robot learning, where the success of RL has been rather limited. We address this issue by building on the general sample efficiency of off-policy algorithms. With nonparametric regression and density estimation methods we construct a nonparametric Bellman equation in a principled manner, which allows us to obtain closed-form estimates of the value function, and to analytically express the full policy gradient. We provide a theoretical analysis of our estimate to show that it is consistent under mild smoothness assumptions and empirically show that our approach has better sample efficiency than state-of-the-art policy gradient methods.

==> experiments/Cartpole_random.tex <==
\begin{figure}[t]
\begin{centering}
    \centering
    \includegraphics[scale=0.6]{figures/experiments/cartpole_randomwalk_samplesize.pdf}
    \caption[Returns in the Cartpole stabilization environment with randomly sampled data]{\textbf{Returns in the Cartpole stabilization environment with randomly sampled data} This plot compares the return obtained by NOPG and typical on- and off-policy algorithms in the CartPole task, as a function of the number of collected samples. NOPG's performance surpasses other algorithms by at least an order of magnitude. The TRPO and DDPG curves start at $5 \cdot 10^2$ samples because to accelerate training we only evaluate these algorithms after collecting every other $5 \cdot 10^2$ samples. The solid line represents the mean and the shaded area the 95\% confidence interval of 10 runs. The details used in this experiment are presented in \tabref{tab:cartpole_random_configs}.}

    \label{fig:cartpole_random}
\end{centering}
\end{figure}


==> experiments/Cartpole_real.tex <==
\begin{figure}[t]
\begin{centering}
    \centering
    \includegraphics[scale=0.5]{figures/experiments/cartpole_real.png}
    \caption[Evaluation of a policy optimized with NOPG-S in the real CartPole system]{\textbf{Evaluation of a policy optimized with NOPG-S in the real CartPole system} This stream of figures (left to right, top to bottom ordering) shows the application of a policy learned in simulation with NOPG-S in the real CartPole environment. The policy was trained using 1500 data points from trajectories with actions randomly sampled from a uniform distribution. Although a compliant policy can be learned with less samples, we found its actions alternated between very low and high signals, leading to very rough movements. We noticed that using more samples solved this problem.}
    \label{fig:cartpole_real}
\end{centering}
\end{figure}


==> experiments/Environments_schematics.tex <==
\begin{figure}[t]
\begin{centering}
    \begin{subfigure}{0.33\textwidth}
      \centering
      \includegraphics[scale=0.5]{figures/experiments/Pendulum_schematic.pdf}
      \caption{Pendulum}
      \label{fig:pendulum_schematic}
    \end{subfigure}%
    \begin{subfigure}{0.33\textwidth}
      \centering
      \includegraphics[scale=0.5]{figures/experiments/CartPole_schematic.pdf}
      \caption{CartPole}
      \label{fig:cartpole_schematic}
    \end{subfigure}
    \begin{subfigure}{0.33\textwidth}
      \centering
      \includegraphics[scale=0.5]{figures/experiments/MountainCar_schematic.pdf}
      \caption{MountainCar}
      \label{fig:mountaincar_schematic}
    \end{subfigure}    
    
    \caption[Environment schematics]{\textbf{Environment schematics} These figures depict the environments used in the experiments.}
    
    \label{fig:environment_schematics}
\end{centering}
\end{figure}

==> experiments/MountainCar_phase_portrait.tex <==
\begin{figure}[t]
\begin{centering}
    \begin{subfigure}{0.5\textwidth}
      \centering
      \includegraphics[scale=0.5]{figures/experiments/MountainCar_V_mu_0.pdf}
      \caption{Before any policy update}
      \label{fig:mountaincar_phase_portrait_a}
    \end{subfigure}%
    \begin{subfigure}{0.5\textwidth}
      \centering
      \includegraphics[scale=0.5]{figures/experiments/MountainCar_V_mu_251.pdf}
      \caption{After 251 policy updates}
      \label{fig:mountaincar_phase_portrait_b}
    \end{subfigure}
    
    \caption[Phase portrait of the value function and state distribution for the MountainCar experiment]{\textbf{Phase portrait of the value function and state distribution for the MountainCar experiment} The plots show the value function and state distribution estimates in the MountainCar environment using NOPG-D. The two leftmost plots show the estimates before any policy update and the rightmost after 251 updates. NOPG-D was trained with 4 trajectories provided by a human demonstrator with the details presented in \tabref{tab:mountaincar_configs}.}
    
    \label{fig:mountaincar_phase_portrait}
\end{centering}
\end{figure}


==> experiments/MountainCar_samplesize.tex <==
\begin{figure}[t]
\begin{centering}
    \centering
    \includegraphics[scale=0.6]{figures/experiments/mountaincar_samplesize.pdf}
    \caption[Returns in the MountainCar environment with varying number of trajectories]{\textbf{Returns in the MountainCar environment with varying number of trajectories} This plot shows the returns obtained by NOPG-D and NOPG-S as a function of the number of trajectories (roughly each trajectory corresponds to 450 samples). The human baseline corresponds to the average return in the human demonstrations and is depicted by the dashed line. The solid line represents the mean and the shaded area the 95\% confidence interval of 10 runs. The details used in this experiment are presented in \tabref{tab:mountaincar_configs}.}
    \label{fig:mountaincar_samplesize}
\end{centering}
\end{figure}


==> experiments/MountainCar_trajectory.tex <==
\begin{figure}[t]
\begin{centering}
    \centering
    \includegraphics[scale=0.6]{figures/experiments/MountainCar_trajectories.pdf}
    \caption[Trajectories in the state space of the MountainCar environment]{\textbf{Trajectories in the state space of the MountainCar environment} This figure shows two trajectories from evaluation runs of NOPG-D in the MountainCar environment. Trajectory's $1$ return is $-79$ and trajectory's $2$ is $-139$. The crosses denote the starting states and the circles the final states. The dashed vertical line at $x=-0.45$ depicts the goal state. The policy used was optimized with NOPG-D trained on 4 trajectories provided by a human demonstrator with the details presented in \tabref{tab:mountaincar_configs}.}
    \label{fig:mountaincar_trajectories}
\end{centering}
\end{figure}


==> experiments/Pendulum_phase_portrait.tex <==
\begin{figure}[t]
\begin{centering}
    \begin{subfigure}{0.5\textwidth}
      \centering
      \includegraphics[scale=0.5]{figures/experiments/Pendulum_V_mu_0.pdf}
      \caption{Before any policy update}
      \label{fig:pendulum_phase_portrait_a}
    \end{subfigure}%
    \begin{subfigure}{0.5\textwidth}
      \centering
      \includegraphics[scale=0.5]{figures/experiments/Pendulum_V_mu_301.pdf}
      \caption{After 301 policy updates}
      \label{fig:pendulum_phase_portrait_b}
    \end{subfigure}
    
    \caption[Phase portrait of the value function and state distribution for the Pendulum environment]{\textbf{Phase portrait of the value function and state distribution for the Pendulum environment} The plots show the value function and state distribution estimates in the Pendulum environment using NOPG-D, with a uniformly sampled data. The two leftmost plots show the estimates before any policy update and the rightmost after 301 updates. In this experiment, data was collected uniformly from a grid of state-action pairs (30 angles, 30 angular velocities, 2 actions) and NOPG-D trained with the details presented in \tabref{tab:pendulum_uniform_configs}.}
    
    \label{fig:pendulum_phase_portrait}
\end{centering}
\end{figure}


==> experiments/Pendulum_random.tex <==
\begin{figure}[t]
\begin{centering}
    \centering
    \includegraphics[scale=0.6]{figures/experiments/pendulum_randomwalk_samplesize.pdf}
    \caption[Returns in the Pendulum environment with randomly sampled data]{\textbf{Returns in the Pendulum environment with randomly sampled data} This plot compares the return obtained by NOPG and typical on- and off-policy algorithms in the Pendulum task, as a function of the number of collected samples. NOPG's performance surpasses other algorithms by at least an order of magnitude. The TRPO and DDPG curves start at $10^3$ samples because to accelerate training we only evaluate these algorithms after collecting every other $10^3$ samples. The solid line represents the mean and the shaded area the 95\% confidence interval of 10 runs. The details used in this experiment are presented in \tabref{tab:pendulum_random_configs}.}
    \label{fig:pendulum_random}
\end{centering}
\end{figure}


==> experiments/Pendulum_uniform.tex <==
\begin{figure}[t]
\begin{centering}
    \centering
    \includegraphics[scale=0.7]{figures/experiments/pendulum_uniform_samplesize.pdf}
    \caption[Returns in the Pendulum environment with uniform sampling]{\textbf{Returns in the Pendulum environment with uniform sampling} This box plot shows the return obtained by NOPG-D and NOPG-S as a function of the dataset size with samples from an uniform grid. The error bars show the results of 10 trials. The datasets' details are found in \tabref{tab:pendulum_uniform}.}
    \label{fig:pendulum_uniform}
\end{centering}
\end{figure}





==> experiments/Pendulum_uniform_table.tex <==
\begin{table}[ht]
\begin{center}
    \begin{tabular}{r r r}
        Sample size & NOPG-D & NOPG-S \\ \hline
        200  & $-3794.9 \pm 11.9$ & $-3788.5 \pm 00.9$  \\
        450  & $-576.3  \pm 03.1$  & $-594.1  \pm 39.8$ \\
        800  & $-572.3  \pm 02.3$  & $-572.8  \pm 03.9$ \\
        1250 & $-567.9  \pm 03.2$  & $-564.2  \pm 01.6$ \\
        1800 & $-472.0  \pm 28.8$  & $-457.9  \pm 26.0$ \\
        3200 & $-415.4  \pm 00.7$  & $-428.0  \pm 26.9$ \\
        \hline
    \end{tabular}
\end{center}

    \caption[Returns in the Pendulum environment with uniform sampling]{\textbf{Returns in the Pendulum environment with uniform sampling} This table presents the returns obtained by NOPG-D and NOPG-S as a function of the dataset size with samples from an uniform grid. Depicted are the mean and 95\% confidence intervals of 10 trials. The datasets' details are found in \tabref{tab:pendulum_uniform}.}
    \label{tab:pendulum_uniform_results}
\end{table}


==> plots/NOPG-D.tex <==
% This file was created by matplotlib2tikz v0.6.18.
\begin{tikzpicture}

\definecolor{color0}{rgb}{1,0.647058823529412,0}

\begin{axis}[
width=\figurewidth,
height=\figureheight,
tick align=outside,
tick pos=left,
title={NOPG-D},
x grid style={white!69.01960784313725!black},
xlabel={Dataset size (samples)},
yticklabel  style={font=\scriptsize},
xticklabel  style={font=\scriptsize},
ylabel style={rotate=-90},
xmin=0.5, xmax=7.5,
xtick={1,2,3,4,5,6,7},
xticklabels={10,50,100,250,500,1000,1500},
y grid style={white!69.01960784313725!black},
ylabel={$J_{\pi}$},
ymin=-0.487, ymax=209.547
]
\addplot [black, forget plot]
table [row sep=\\]{%
1	9.34 \\
1	9.14 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
1	12.3 \\
1	15.62 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
0.875	9.14 \\
1.125	9.14 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
0.875	15.62 \\
1.125	15.62 \\
};
\addplot [black, mark=*, mark size=3, mark options={solid,fill opacity=0}, only marks, forget plot]
table [row sep=\\]{%
1	20.94 \\
1	64.54 \\
1	27.22 \\
1	38.08 \\
1	25.34 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
2	9.97 \\
2	9.24 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
2	48 \\
2	92.52 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
1.875	9.24 \\
2.125	9.24 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
1.875	92.52 \\
2.125	92.52 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
3	9.48 \\
3	9.06 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
3	43.545 \\
3	68.4 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
2.875	9.06 \\
3.125	9.06 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
2.875	68.4 \\
3.125	68.4 \\
};
\addplot [black, mark=*, mark size=3, mark options={solid,fill opacity=0}, only marks, forget plot]
table [row sep=\\]{%
3	101.86 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
4	12.07 \\
4	9.1 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
4	82.795 \\
4	181.56 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
3.875	9.1 \\
4.125	9.1 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
3.875	181.56 \\
4.125	181.56 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
5	56.945 \\
5	9.34 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
5	129.605 \\
5	200 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
4.875	9.34 \\
5.125	9.34 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
4.875	200 \\
5.125	200 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
6	99.21 \\
6	53.32 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
6	141.64 \\
6	200 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
5.875	53.32 \\
6.125	53.32 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
5.875	200 \\
6.125	200 \\
};
\addplot [black, mark=*, mark size=3, mark options={solid,fill opacity=0}, only marks, forget plot]
table [row sep=\\]{%
6	9.42 \\
6	9.44 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
7	104.495 \\
7	9.36 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
7	175.07 \\
7	200 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
6.875	9.36 \\
7.125	9.36 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
6.875	200 \\
7.125	200 \\
};
\path [draw=black, fill=color0] (axis cs:0.75,9.34)
--(axis cs:1.25,9.34)
--(axis cs:1.25,12.3)
--(axis cs:0.75,12.3)
--(axis cs:0.75,9.34)
--cycle;

\path [draw=black, fill=color0] (axis cs:1.75,9.97)
--(axis cs:2.25,9.97)
--(axis cs:2.25,48)
--(axis cs:1.75,48)
--(axis cs:1.75,9.97)
--cycle;

\path [draw=black, fill=color0] (axis cs:2.75,9.48)
--(axis cs:3.25,9.48)
--(axis cs:3.25,43.545)
--(axis cs:2.75,43.545)
--(axis cs:2.75,9.48)
--cycle;

\path [draw=black, fill=color0] (axis cs:3.75,12.07)
--(axis cs:4.25,12.07)
--(axis cs:4.25,82.795)
--(axis cs:3.75,82.795)
--(axis cs:3.75,12.07)
--cycle;

\path [draw=black, fill=color0] (axis cs:4.75,56.945)
--(axis cs:5.25,56.945)
--(axis cs:5.25,129.605)
--(axis cs:4.75,129.605)
--(axis cs:4.75,56.945)
--cycle;

\path [draw=black, fill=color0] (axis cs:5.75,99.21)
--(axis cs:6.25,99.21)
--(axis cs:6.25,141.64)
--(axis cs:5.75,141.64)
--(axis cs:5.75,99.21)
--cycle;

\path [draw=black, fill=color0] (axis cs:6.75,104.495)
--(axis cs:7.25,104.495)
--(axis cs:7.25,175.07)
--(axis cs:6.75,175.07)
--(axis cs:6.75,104.495)
--cycle;

\addplot [black, forget plot]
table [row sep=\\]{%
0.75	9.42 \\
1.25	9.42 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
1.75	22 \\
2.25	22 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
2.75	20.77 \\
3.25	20.77 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
3.75	46.82 \\
4.25	46.82 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
4.75	92.18 \\
5.25	92.18 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
5.75	123.92 \\
6.25	123.92 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
6.75	153.67 \\
7.25	153.67 \\
};
\end{axis}

\end{tikzpicture}

==> plots/NOPG-S.tex <==
% This file was created by matplotlib2tikz v0.6.18.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.564705882352941,0.933333333333333,0.564705882352941}

\begin{axis}[
width=\figurewidth,
height=\figureheight,
tick align=outside,
tick pos=left,
title={NOPG-S},
x grid style={white!69.01960784313725!black},
xlabel={Dataset size (samples)},
yticklabel  style={font=\tiny},
xticklabel  style={font=\tiny},
ylabel style={rotate=-90},
xmin=0.5, xmax=7.5,
xtick={1,2,3,4,5,6,7},
xticklabels={10,50,100,250,500,1000,1500},
y grid style={white!69.01960784313725!black},
ylabel={$J_{\pi}$},
ymin=-0.382, ymax=209.542
]
\addplot [black, forget plot]
table [row sep=\\]{%
1	9.34 \\
1	9.16 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
1	10.695 \\
1	11.74 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
0.875	9.16 \\
1.125	9.16 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
0.875	11.74 \\
1.125	11.74 \\
};
\addplot [black, mark=*, mark size=3, mark options={solid,fill opacity=0}, only marks, forget plot]
table [row sep=\\]{%
1	26.6 \\
1	12.94 \\
1	14.9 \\
1	18.98 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
2	9.45 \\
2	9.16 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
2	50.225 \\
2	110.52 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
1.875	9.16 \\
2.125	9.16 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
1.875	110.52 \\
2.125	110.52 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
3	31.845 \\
3	9.3 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
3	72.51 \\
3	106.94 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
2.875	9.3 \\
3.125	9.3 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
2.875	106.94 \\
3.125	106.94 \\
};
\addplot [black, mark=*, mark size=3, mark options={solid,fill opacity=0}, only marks, forget plot]
table [row sep=\\]{%
3	136.74 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
4	36.92 \\
4	9.24 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
4	88.775 \\
4	137.26 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
3.875	9.24 \\
4.125	9.24 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
3.875	137.26 \\
4.125	137.26 \\
};
\addplot [black, mark=*, mark size=3, mark options={solid,fill opacity=0}, only marks, forget plot]
table [row sep=\\]{%
4	200 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
5	49.39 \\
5	10.1 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
5	116.725 \\
5	189.88 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
4.875	10.1 \\
5.125	10.1 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
4.875	189.88 \\
5.125	189.88 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
6	77.135 \\
6	9.36 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
6	141.23 \\
6	200 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
5.875	9.36 \\
6.125	9.36 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
5.875	200 \\
6.125	200 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
7	104.495 \\
7	49.86 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
7	160.685 \\
7	200 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
6.875	49.86 \\
7.125	49.86 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
6.875	200 \\
7.125	200 \\
};
\path [draw=black, fill=color0] (axis cs:0.75,9.34)
--(axis cs:1.25,9.34)
--(axis cs:1.25,10.695)
--(axis cs:0.75,10.695)
--(axis cs:0.75,9.34)
--cycle;

\path [draw=black, fill=color0] (axis cs:1.75,9.45)
--(axis cs:2.25,9.45)
--(axis cs:2.25,50.225)
--(axis cs:1.75,50.225)
--(axis cs:1.75,9.45)
--cycle;

\path [draw=black, fill=color0] (axis cs:2.75,31.845)
--(axis cs:3.25,31.845)
--(axis cs:3.25,72.51)
--(axis cs:2.75,72.51)
--(axis cs:2.75,31.845)
--cycle;

\path [draw=black, fill=color0] (axis cs:3.75,36.92)
--(axis cs:4.25,36.92)
--(axis cs:4.25,88.775)
--(axis cs:3.75,88.775)
--(axis cs:3.75,36.92)
--cycle;

\path [draw=black, fill=color0] (axis cs:4.75,49.39)
--(axis cs:5.25,49.39)
--(axis cs:5.25,116.725)
--(axis cs:4.75,116.725)
--(axis cs:4.75,49.39)
--cycle;

\path [draw=black, fill=color0] (axis cs:5.75,77.135)
--(axis cs:6.25,77.135)
--(axis cs:6.25,141.23)
--(axis cs:5.75,141.23)
--(axis cs:5.75,77.135)
--cycle;

\path [draw=black, fill=color0] (axis cs:6.75,104.495)
--(axis cs:7.25,104.495)
--(axis cs:7.25,160.685)
--(axis cs:6.75,160.685)
--(axis cs:6.75,104.495)
--cycle;

\addplot [black, forget plot]
table [row sep=\\]{%
0.75	9.48 \\
1.25	9.48 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
1.75	21.07 \\
2.25	21.07 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
2.75	53.37 \\
3.25	53.37 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
3.75	51.85 \\
4.25	51.85 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
4.75	64.98 \\
5.25	64.98 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
5.75	107.64 \\
6.25	107.64 \\
};
\addplot [black, forget plot]
table [row sep=\\]{%
6.75	142.11 \\
7.25	142.11 \\
};
\end{axis}

\end{tikzpicture}
